SpectralGaussians: Semantic, spectral 3D Gaussian splatting for multi-spectral scene representation, visualization and analysis

We propose a novel cross-spectral rendering framework based on 3D Gaussian Splatting (3DGS) that generates realistic and semantically meaningful splats from registered multi-view spectrum and segmentation maps. This extension enhances the representation of scenes with multiple spectra, providing insights into the underlying materials and segmentation. We introduce an improved physically-based rendering approach for Gaussian splats, estimating reflectance and lights per spectra, thereby enhancing accuracy and realism. In a comprehensive quantitative and qualitative evaluation, we demonstrate the superior performance of our approach with respect to other recent learning-based spectral scene representation approaches (i.e., XNeRF and SpectralNeRF) as well as other non-spectral state-of-the-art learning-based approaches. Our work also demonstrates the potential of spectral scene understanding for precise scene editing techniques like style transfer, inpainting, and removal. Thereby, our contributions address challenges in multi-spectral scene representation, rendering, and editing, offering new possibilities for diverse applications.

==> text/abstract.tex <==
\begin{abstract}
We propose a novel cross-spectral rendering framework based on 3D Gaussian Splatting (3DGS) that generates realistic and semantically meaningful splats from registered multi-view spectrum and segmentation maps. This extension enhances the representation of scenes with multiple spectra, providing insights into the underlying materials and segmentation. We introduce an improved physically-based rendering approach for Gaussian splats, estimating reflectance and lights per spectra, thereby enhancing accuracy and realism.
%
In a comprehensive quantitative and qualitative evaluation, we demonstrate the superior performance of our approach with respect to other recent learning-based spectral scene representation approaches (i.e., XNeRF and SpectralNeRF) as well as other non-spectral state-of-the-art learning-based approaches.
%
Our work also demonstrates the potential of spectral scene understanding for precise scene editing techniques like style transfer, inpainting, and removal. Thereby, our contributions address challenges in multi-spectral scene representation, rendering, and editing, offering new possibilities for diverse applications.
%
%Additionally, we provide a comprehensive quantitative and qualitative analysis, validating the accuracy and fidelity of our method.
\end{abstract}
% Each keyword is seperated by \sep
\begin{keywords}
Computer graphics \sep Deep learning \sep Spectral imaging \sep 3D reconstruction \sep 3D Gaussian splatting \sep Appearance modeling \sep Scene understanding and editing \sep Novel view synthesis
\end{keywords}


==> text/our_macros.tex <==
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\etal{et~al.\ }
\def\wrt{w.r.t.\ }
%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\argmin}{argmin}

%\usepackage{tabularx}
%\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}
%\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
%\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

\usepackage[normalem]{ulem}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\added}[1]{\textcolor{blue}{#1}}
\newcommand{\mwrevision}[2]{{\color{red}\sout{#1}}{\color{green}\uwave{#2}}}
\newcommand{\neilrevision}[2]{{\color{red}\sout{#1}}{\color{blue}\uwave{#2}}}
